3D Macro Physics and Light Odd-Z Element Production in O-C Shell Mergers: Implications for $^{40}\mathrm{K}$ production and radiogenic heating inventories of rocky exoplanets

The light odd-Z elements P, Cl, K, and Sc are underproduced in galactic chemical evolution models compared to spectroscopic observations of stars in the Milky Way. The most promising solution to this puzzle is that some massive stars experience O-C shell mergers boosting their yields through dynamic, convective-reactive nucleosynthesis. We report how convective macro physics based on 3D $4\pi$ hydrodynamic simulations impacts production in the O shell by post-processing the $\mathrm{M_{ZAMS}}=15~\mathrm{M_\odot}$ $Z=0.02$ model from the NuGrid dataset. We explore a mixing downturn, boosted velocities, reduced ingestion rate, and convective quenching. Across 24 mixing cases, the pre-explosive yields for [P/Fe], [Cl/Fe], [K/Fe], and [Sc/Fe] are modified by $[-0.33,0.23]~\mathrm{dex}$, $[-0.84,0.64]~\mathrm{dex}$, $[-0.78,1.48]~\mathrm{dex}$, and $[-0.36,1.29]~\mathrm{dex}$, respectively. Cases with a convective downturn with the fastest ingestion rate have the largest enhancement, and production is non-monotonic with boosted velocities. Which reactions are most important for the convective-reactive element production pathways depends on the mixing. We parameterize production of $^{40}\mathrm{K}$ ($t_{1/2} = 1.248~\mathrm{Gyr}$), an important radiogenic heat source for younger ($2{-}3~\mathrm{Gyr}$) rocky planets and find a yield variation exceeding three orders of magnitude. This range of initial abundances for $^{40}\mathrm{K}$ implies the early geodynamic behaviour of silicate mantles in rocky planets can differ greatly from that of Earth. These results underscore the importance of investigating the 3D macro physics of shell merger convection through hydrodynamic simulations to develop a predictive understanding of the origin and variability of the light odd-Z elements and the $^{40}\mathrm{K}/\mathrm{K}$ ratio in planet host stars.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
\newcommand{\vort}{\ensuremath{|\curl u|}}
\newcommand{\vortsq}{\ensuremath{\vort^2}}
% end vectors.tex

